Some Bibliographical References on Intonation and Intonational Meaning

A by-no-means-complete collection of references for those interested in intonational meaning, with other miscellaneous references on intonation included. Additional references are welcome, and should be sent to julia@research.att.com.

==> 9405003.2 <==
@string{garland="Garland Publishing, Inc."}
@string{jml="Journal of Memory and Language."}
@string{foris="Foris Publications"}
@string{sv="Springer-Verlag"}
@string{stanford="Stanford University"}
@string{stanfordp="Stanford University Press"}
@string{erlbaum="Lawrence Erlbaum Associates"}
@string{jasa="Journal of the Acoustical Society of America"}
@string{escol="Eastern States Conference on Linguistics"}
@string{aaai="American Association for Artificial Intelligence"}
@string{lang="Language"}
@string{reidel="D. Reidel Publishing Company"}
@string{upenn="University of Pennsylvania"}
@string{mit="The Massachusetts Institute of Technology"}
@string{mitp="MIT Press"}
@string{ph="Prentice-Hall"}
@string{cuny="City University of New York"}
@string{ucla="University of California at Los Angeles"}
@string{ut="The University of Texas at Austin"}
@string{cls="Chicago Linguistic Society"}
@string{ny="New York"}
@string{chi="Chicago"}
@string{cambma="Cambridge MA"}
@string{cambuk="Cambridge UK"}
@string{cup="Cambridge University Press"}
@string{dord="Dordrecht"}
@string{ac="Academic Press"}
@string{chip="The University of Chicago Press"}
@string{li="Linguistic Inquiry"}
@string{s&s="Syntax and Semantics"}
@string{cogsci="Cognitive Science"}
@string{cogpsy="Cognitive Psychology"}
@string{dec="December"}
@string{acl="Association for Computational Linguistics"}
@string{ijcai="International Joint Conference on Artificial Intelligence"}
@string{coling="International Conference on Computational
@string{coling84="Proceedings of Coling84"}
@string{coling86="Proceedings of the 11th International Conference on
Computational
@string{coling88="Proceedings of the 12th International Conference on
Computational Linguistics"}
@string{coling90="Papers Presented to the 13th International
@string{coling92="Papers Presented to the 15th International Conference on
Computational Linguistics"}
@article{Akmajian70,
	key="Akmajian",
	author="Akmajian, Adrian and Jackendoff, Ray",
	title="Coreferentiality and Stress",
	journal=li,
	volume="1",
	number="1",
	year="1970",
	pages="124-126"}

@Article{Allerton79,
  author = 	"Allerton, D. and Cruttenden, A.",
  title = 	"Three Reasons for Accenting a Definite Subject",
  journal = 	"Journal of Linguistics",
  year = 	"1979",
  volume = 	"15",
  number = 	"1",
  pages = 	"49-53",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Altenberg87,
  author = 	"Altenberg, Bengt",
  title = 	"Prosodic Patterns in Spoken {E}nglish:  Studies in the
		 Correlation between Prosody and Grammar for
		 Text-to-Speech Conversion",
  publisher = 	"Lund University Press",
  year = 	"1987",
  OPTeditor = 	"",
  volume = 	"76",
  series = 	"Lund Studies in {E}nglish",
  address = 	"Lund",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@inproceedings{Anderson84,
	key="Anderson",
	author="Anderson, Mark D. and Pierrehumbert, Janet B. and Liberman, Mark Y.",
	title="Synthesis by Rule of {E}nglish Intonation Patterns",
	booktitle="Proceedings of the International Conference on
Acoustics, Speech, and Signal Processing",
	organization="ICASSP84",
	address="San Diego",
	year="1984",
	pages="2.8.1-2.8.4",
	volume="1"}

@Proceedings{Autrans90,
  title = 	"Proceedings of the {E}uropean Speech Communication
		 Association
Workshop on Speech Synthesis",
  year = 	"1989",
  editor = 	"Benoit, Christian and Gerard Bailly",
  OPTpublisher = 	"",
  organization = 	"{E}uropean Speech Communication Association",
  address = 	"Autrans",
  month = 	"September",
  OPTnote = 	"Institut de la Communication Parlee, Grenoble"
}

@InProceedings{Avesani88,
  author = 	"Avesani, Cinzia and Vayra, Mario",
  title = 	"Discorso, Segmenti di Discorso e un{'} Ipotesi
		 sull{'} Intonazione",
  booktitle = 	"Att del Convegno Internazionale {"}Sull'Interpunzione{"}",
  year = 	"1988",
  OPTeditor = 	"",
  OPTpages = 	"",
  OPTorganization = 	"",
  OPTpublisher = 	"",
  address = 	"Florence",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Unpublished{Ayers92,
  author = 	"Ayers, Gayle M.~",
  title = 	"Discourse Functions of Pitch Range in Spontaneous and
		 Read Speech",
  note = 	"Presented at the Linguistic Society of America Annual Meeting",
  year = 	"1992",
  address =     "Philadelphia",
  OPTmonth = 	""
}

@PhDThesis{Baart87,
  author = 	"Baart, J.~L.~G.",
  title = 	"Focus, Syntax and Accent Placement",
  school = 	"University of Leyden",
  year = 	"1987",
  address = 	"Leyden",
  OPTmonth = 	"",
  OPTnote = 	""
}

@article{Bachenko90,
	author="Bachenko, J. and Fitzpatrick, E.",
	title="A Computational Grammar of Discourse-Neutral Prosodic
		 Phrasing in {E}nglish",
        year="1990",
	journal="Computational Linguistics",
        volume="16",
        number="3",
        pages="155-170"

}

@Article{Ball77,
  author = 	"Ball, C.~N. and Prince, E.~ F.",
  title = 	"A Note on Stress and Presupposition",
  journal = 	"Linguistic Inquiry",
  year = 	"1977",
  volume = 	"8",
  number = 	"3",
  pages = 	"585",
  OPTmonth = 	"",
  OPTnote = 	""
}

@phdthesis{Bardovi83a,
	key="Bardovi",
	author="Bardovi-Harlig, Kathleen",
	title="A Functional Approach to {E}nglish Sentence Stress",
	school="University of Chicago",
	year="1983",
	address="Chicago IL"}

@InProceedings{Bardovi83b,
  author = 	"Bardovi-Harlig, K.",
  title = 	"Pronouns:  When `Given' and `New' Coincide",
  booktitle = 	"Papers from the 18th Regional Meeting",
  year = 	"1983",
  OPTeditor = 	"",
  OPTpages = 	"",
  organization = 	cls,
  OPTpublisher = 	"",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Beach91,
  author = 	"Beach, Cheryl",
  title = 	"The Interpretation of Prosodic Patterns at Points of
		 Syntactic Structure Ambiguity:  Evidence for Cue
		 Trading Relations",
  journal = 	jml,
  year = 	"1991",
  volume = 	"30",
  OPTnumber = 	"",
  pages = 	"644-663",
  OPTmonth = 	"",
  OPTnote = 	""
}

@inproceedings{Beckman86a,
	key="Beckman",
	author="Beckman, M. and Pierrehumbert, J.",
	title="{J}apanese Prosodic Phrasing and Intonation Synthesis",
	booktitle="Proceedings of the 24th Annual Meeting",
	organization=acl,
	address=ny,
	year="1986",
	pages="173-180"}

@article{Beckman86b,
	key="Beckman",
	author="Beckman, Mary and  Pierrehumbert, Janet",
	title="Intonational Structure in {J}apanese and {E}nglish",
	journal="Phonology Yearbook",
	volume="3",
	year="1986",
	pages="15-70"}

@Book{Beckman86c,
  author = 	"Beckman, Mary",
  title = 	"Stress and Non-Stress Accent",
  publisher = 	foris,
  year = 	"1986",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  OPTaddress = 	"",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@phdthesis{Bing79b,
	key="Bing",
	author="Bing, Janet",
	title="Aspects of {E}nglish Prosody",
	address="Amherst MA",
	school="University of Massachusetts at Amherst",
        note="Distributed by the Indiana University Linguistics Club",
	year="1979"}

@Article{Bolinger51,
  author = 	"Bolinger, Dwight",
  title = 	"Intonation:  Levels versus Configurations",
  journal = 	"Word",
  year = 	"1951",
  volume = 	"7",
  number = 	"1",
  pages = 	"199-210",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Bolinger58,
	Author="Bolinger, Dwight",
	Key="Bolinger",
	Title="A Theory of Pitch Accent in {E}nglish",
	Journal="Word",
	Volume="14",
	Pages="109-149",
	Year="1958"}

@Article{Bolinger61,
  author = 	"Bolinger, Dwight",
  title = 	"Contrastive Accent and Contrastive Stress",
  journal = 	"Language",
  year = 	"1961",
  volume = 	"37",
  OPTnumber = 	"",
  pages = 	"83-96",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Bolinger72a,
  author =      "Bolinger, Dwight",
  title = 	"Accent is Predictable (If You're a Mindreader)",
  journal = 	"Language",
  year = 	"1972",
  volume = 	"48",
  OPTnumber = 	"",
  pages = 	"633-644",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Bolinger82,
  author = 	"Bolinger, Dwight",
  title = 	"The Network Tone of Voice",
  journal = 	"Journal of Broadcasting",
  year = 	"1982",
  volume = 	"26",
  OPTnumber = 	"",
  pages = 	"725-728",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Bolinger86,
  author = 	"Bolinger, Dwight",
  title = 	"Intonation and Its Parts:  Melody in Spoken {E}nglish",
  publisher = 	"Stanford University Press",
  year = 	"1986",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Palo Alto CA",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Bolinger89,
  author = 	"Bolinger, Dwight",
  title = 	"Intonation and Its Uses:  Melody in Grammar and Discourse",
  publisher = 	"Edward Arnold",
  year = 	"1989",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"London",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Bouton82,
  author = 	"Bouton, Lawrence F.",
  title = 	"Stem Polarity and Tag Intonation in the Derivation of
		 the Imperative Tag",
  booktitle = 	"Papers from the Parasession on Nondeclaratives",
  year = 	"1982",
  editor = 	"Schneider, Robinson and Tuite, Kevin and Chametzky, Robert",
  pages = 	"23-42",
  organization = 	"Chicago Linguistic Society",
  OPTpublisher = 	"",
  address = 	"Chicago",
  OPTmonth = 	"",
  OPTnote = 	""
}

@book{Brazil80,
	key="Brazil",
	author="Brazil, D. and Coulthard, M. and Johns, C.",
	title="Discourse Intonation and Language Teaching",
	publisher="Longman",
	address="London",
	year="1980"}

@Article{Bresnan71,
  author = 	"Bresnan, Joan",
  title = 	"Sentence Stress and Syntactic Transformations",
  journal = 	"Language",
  year = 	"1971",
  volume = 	"47",
  OPTnumber = 	"",
  pages = 	"257-281",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Bruce90,
  author = 	"Bruce, G. and Granstrom, B. and House, D.",
  title = 	"Prosodic Phrasing in {S}wedish Speech Synthesis",

  booktitle = 	"Proceedings of the {E}uropean Speech Communication
		 Association
Workshop on Speech Synthesis",
  year = 	"1990",
  organization = 	"{E}uropean Speech Communication Association",
  address = 	"Autrans, France",
  month = 	"September",
  pages = 	"125-128",
  OPTnote = 	""
}

@article{Butterworth75,
	key="Butterworth",
	author="Butterworth, B.",
	title="Hesitation and Semantic Planning in Speech",
	journal="Journal of Psycholinguistic Research",
	volume="4",
	year="1975",
	pages="75-87"}

@Article{Butterworth77,
  author = 	"Butterworth, B.",
  title = 	"Speech and Interaction in Sound-Only Communication Channels",
  journal = 	"Semiotica",
  year = 	"1977",
  volume = 	"20",
  number = 	"2",
  pages = 	"81-99",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Buxton83,
  author = 	"Buxton, H.",
  title = 	"Temporal Predictability in the Perception of
		 {E}nglish Speech",
  booktitle =   "Prosody:  Models and Measurements",
  publisher = 	sv,
  year = 	"1983",
  editor = 	"Cutler, A. and Ladd. D.~R",
  pages = 	"111-122",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Berlin",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Cantrall69,
  author = 	"Cantrall, W.",
  title = 	"Pitch, Stress, and Grammatical Relations",
  booktitle = 	"Papers from the 5th Regional Meeting",
  year = 	"1969",
  OPTeditor = 	"",
  OPTpages = 	"12-23",
  organization = 	cls,
  OPTpublisher = 	"",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Cantrall75,
  author = 	"Cantrall, W.",
  title = 	"Favored Structures and Intonational Limitations",
  booktitle = 	"Papers from the Parasession on Functionalism",
  year = 	"1975",
  OPTeditor = 	"",
  OPTpages = 	"36-46",
  organization = 	cls,
  OPTpublisher = 	"",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Carlson83,
  author = 	"Carlson, L.",
  title = 	"Dialogue Games",
  publisher = 	"Reidel",
  year = 	"1983",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  OPTaddress = 	"",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Chafe76,
	Author="Chafe, Wallace",
	Key="Chafe",
	Title="Givenness, Contrastiveness, Definiteness, Subjects, Topics, and Point
of View",
	BookTitle="Subject and Topic",
	Editor="Li, C.",
	Publisher=ac,
pages="25-55",
	Address="New York",
	Year="1976"}

@Article{Cooper77,
  author = 	"Cooper, W.~E. and Sorenson, J.~M.",
  title = 	"Fundamental Frequency Contours at Syntactic Boundaries",
  journal = 	jasa,
  year = 	"1977",
  volume = 	"62",
  number = 	"3",
  pages = 	"683-692",
  month = 	"September",
  OPTnote = 	""
}

@Book{Cooper80,
  author = 	"Cooper, W. and Paccia-Cooper, J.",
  title = 	"Syntax and Speech",
  publisher = 	"Harvard University Press",
  year = 	"1980",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Cambridge MA",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Couper-Kuhlen84,
  author = 	"Couper-Kuhlen, Elizabeth",
  title = 	"A New Look at Contrastive Intonation",
  booktitle = 	"Modes of Interpretation:  Essays Presented to Ernst Leisi",
  publisher = 	"Gunter Narr Verlag",
  year = 	"1984",
  editor = 	"Watts, Richard J. and Weidmann, Urs",
  OPTchapter = 	"",
  pages = 	"137-158",
  address = 	"Tubingen",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Couper-Kuhlen86,
  author = 	"Couper-Kuhlen, Elizabeth",
  title = 	"An Introduction to {E}nglish Prosody",
  publisher = 	"Edward Arnold",
  year = 	"1986",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"London",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Cruttenden86,
  author = 	"Cruttenden, A.",
  title = 	"Intonation",
  publisher = 	"Cambridge University Press",
  year = 	"1986",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Cambridge UK",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@PhDThesis{Cruz-Ferreira83,
  author = 	"Cruz-Ferreira",
  title = 	"Non-Native Comprehension of Intonation Patterns in
		 Portuguese and in {E}nglish",
  school = 	"University of Manchester",
  year = 	"1983",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@book{Crystal69,
	key="Crystal",
	author="Crystal, D.",
	title="Prosodic Systems and Intonation in {E}nglish",
	publisher="Cambridge University Press",
	address="Cambridge UK",
	year="1969"}

@book{Crystal75,
	key="Crystal",
	author="Crystal, D.",
	title="The {E}nglish Tone of Voice:  Essays in
Intonation, Prosody, and Paralanguage",
	publisher="Edward Arnold",
	address="London",
	year="1975"}

@Article{Culicover83,
	Author="Culicover, Peter W. and Michael Rochemont",
	Key="Culicover",
	Title="Stress and Focus in {E}nglish",
	Journal=lang,
	Volume="59",
	Number="1",
	Pages="123-165",
	Month="March",
	Year="1983"}

@InProceedings{Cutler77a,
	Author="Cutler, Anne",
	Key="Cutler",
	Title="The Context-Dependence of `Intonational Meanings'",
	Organization="Chicago Linguistic Society",
	BookTitle="Papers of the Fifth Regional Meeting",
	Address="Chicago",
	Year="1977"}

@Article{Cutler77b,
  author = 	"Cutler, A. and Foss, D.",
  title = 	"On the Role of Sentence Stress in Sentence Processing",
  journal = 	"Language and Speech",
  year = 	"1977",
  volume = 	"20",
  OPTnumber = 	"",
  pages = 	"1-10",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Cutler83a,
  author = 	"Cutler, A and Ladd, D.~R., eds.",
  title = 	"Prosody:  Models and Measurements",
  publisher = 	sv,
  year = 	"1983",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Berlin",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Cutler83b,
  author = 	"Cutler, Anne",
  title = 	"Speakers' Conceptions of the Functions of Prosody",
  booktitle = 	"Prosody:  Models and Measurements",
  publisher = 	sv,
  year = 	"1983",
  editor = 	"Cutler, A. and Ladd, D.~R.",
  OPTchapter = 	"",
  pages = 	"79-92",
  address = 	"Berlin",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{DHouse89,
  author = 	"House, D.",
  title = 	"Automatic Recognition of Prosodic Categories",
  booktitle = 	"Proceedings of the Speech Research '89 International
Conference",
  year = 	"1989",
  editor = 	"Szende, T.",
  pages = 	"347-350",
  OPTorganization = 	"",
  OPTpublisher = 	"",
  address = 	"Budapest",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{DHouse90a,
  author = 	"House, D.",
  title = 	"Tonal Perception in Speech",
  publisher = 	"Lund University Press",
  year = 	"1990",
  OPTeditor = 	"",
  volume = 	"24",
  series = 	"Travaux de l'Institut de Linguistique de Lund",
  address = 	"Lund",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@inproceedings{Danlos86,
	key="Danlos",
	author="Danlos, Laurence and Eric La{P}orte and Francoise Emerard",
	title="Synthesis of Spoken Messages from Semantic Representations",
	organization=coling,
	booktitle=coling86,
	year="1986",
	pages="599-604"}

@inproceedings{Davis88,
	key="Davis",
	author="Davis, J.~ R.~ and Hirschberg, J.~",
	booktitle="Proceedings of the 26th Annual Meeting",
	title="Assigning Intonational Features in Synthesized Spoken
Directions",
	organization=acl,
	address="Buffalo",
	year="1988",
	pages="187-193"
}

@Book{Denes73,
  author = 	"Denes, Peter B.~ and Elliot N.~ Pinson",
  title = 	"The Speech Chain:  The Physics and Biology of Spoken Language",
  publisher = 	"Anchor Press",
  year = 	"1973",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Garden City NY",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Dirksen92,
  author = 	"Dirksen, A.",
  title = 	"Accenting and Deaccenting:  A Declarative Approach",
  booktitle = 	"Proceedings of COLING-92",
  year = 	"1992",
  OPTeditor = 	"",
  pages = 	"865-869",
  OPTorganization = 	"",
  OPTpublisher = 	"",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@PhDThesis{Downing70,
  author = 	"Downing, B.",
  title = 	"Syntactic Structure and Phonological Phrasing in {E}nglish",
  school = 	"University of Texas",
  year = 	"1970",
  address = 	"Austin",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Duncan77,
  author = 	"Duncan, S. and Fiske, D.~W.",
  title = 	"Face to Face Interaction:  Research, Methods and Theory",
  publisher = 	erlbaum,
  year = 	"1982",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Hillsdale NJ",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Edwards88,
  author = 	"Edwards, Jan and Beckman, Mary E.",
  title = 	"Articulatory Timing and the Prosodic Interpretation
		 of Syllable Duration",
  journal = 	"Phonetica",
  year = 	"1988",
  volume = 	"45",
  OPTnumber = 	"",
  pages = 	"156-174",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Enkvist79,
  author = 	"Enkvist, N.",
  title = 	"Marked Focus:  Functions and Constraints",
  booktitle = 	"Studies in {E}nglish Linguistics for Randolph Quirk",
  publisher = 	"Longmans",
  year = 	"1979",
  editor = 	"Greenbaum, S. and Leech, G. and Svartvik, J.",
  OPTchapter = 	"",
  pages = 	"134-152",
  address = 	"London",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Erteschik83,
  author = 	"Erteschik-Shir, Nomi and Lappin, Shalom",
  title = 	"Under Stress:  A Functional Explanation of {E}nglish
		 Sentence Stress",
  journal = 	"Journal of Linguistics",
  year = 	"1983",
  volume = 	"19",
  OPTnumber = 	"",
  pages = 	"419-453",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Ervin-Tripp79,
  author = 	"Ervin-Tripp, S.",
  title = 	"Children's Verbal Turn-Taking",
  booktitle = 	"Developmental Pragmatics",
  publisher = 	ac,
  year = 	"1979",
  editor = 	"Ochs, E. and Shieffelin, B.~B.",
  OPTchapter = 	"",
  pages = 	"391-414",
  address = 	ny,
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Fernald91a,
  author = 	"Fernald, Anne and Claudia Mazzie",
  title = 	"Prosody and Focus in Speech to Infants and Adults",
  journal = 	"Developmental Psychology",
  year = 	"1991",
  volume = 	"27",
  number = 	"2",
  pages = 	"209-221",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Fernald91b,
  author = 	"Fernald, Anne",
  title = 	"Prosody in Speech to Children:  Prelinguistic and
		 Linguistic Functions",
  booktitle = 	"Annals of Child Development",
  publisher = 	"Jessica Kingsley Publishers",
  year = 	"1991",
  editor = 	"R.~Vasta",
  OPTchapter = 	"",
  OPTpages = 	"",
  address = 	"London",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Fowler87,
  author = 	"Fowler, C.~A.~ and J.~ Housum",
  title = 	"Talkers' signaling of {"new"} and {"old"} words in
		 speech and listeners' perception and use of the distinction",
  journal = 	"Journal of Memory and Language",
  year = 	"1987",
  volume = 	"26",
  OPTnumber = 	"",
  pages = 	"489-504",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Fry58,
  author = 	"Fry, D.~B.",
  title = 	"Experiments in the Perception of Stress",
  journal = 	"Language and Speech",
  year = 	"1958",
  volume = 	"1",
  OPTnumber = 	"",
  pages = 	"126-152",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Fry79,
  author = 	"Fry, D.~ B.~",
  title = 	"The Physics of Speech",
  publisher = 	"Cambridge University Press",
  year = 	"1979",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Cambridge UK",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Fuchs80,
  author = 	"Fuchs, A.",
  title = 	"Accented Subjects in `All-New' Utterances",
  booktitle = 	"Wege zur Universalienforschung:
		 sprachwissenschaftliche Beitrage zum 60.",
  publisher = 	"Narr",
  year = 	"1980",
  editor = 	"Brettschneider, G. and Lehmann, C.",
  OPTchapter = 	"",
  OPTpages = 	"",
  address = 	"Tubingen",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Fuchs84,
  author = 	"Fuchs, A.",
  title = 	"Deaccenting and Default Accent",
  booktitle = 	"Intonation, Accent and Rhythm",
  publisher = 	"Walter de Gruyter",
  year = 	"1984",
  editor = 	"D.~Gibbon and H. ~Richter",
  pages = 	"134-164",
  address = 	"Berlin",
  OPTmonth = 	"",
  OPTnote = 	""
}

@book{GBrown80,
	key="Brown",
	author="Brown, G. and Currie, K. and Kenworthy, J.",
	title="Questions of Intonation",
	publisher="University Park Press",
	address="Baltimore",
	year="1980"}

@InCollection{GBrown83a,
  author = 	"Brown, G.",
  title = 	"Prosodic Structure and the Given/New Distinction",
  booktitle = 	"Prosody:  Models and Measurements",
  publisher = 	"Springer Verlag",
address = "Berlin",
  year = 	"1983",
  editor = 	"D.~R. Ladd and A. Cutler",
  OPTchapter = 	"",
  pages = 	"67-78",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{GBrown83b,
  author = 	"Brown, G. and G.~ Yule",
  title = 	"Discourse Analysis",
  publisher = 	"Cambridge University Press",
  year = 	"1983",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Cambridge UK",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Garding83,
  author = 	"Garding, Eva",
  title = 	"A Genertive Model of Intonation",
  booktitle = 	"Prosody:  Models and Measurements",
  publisher = 	sv,
  year = 	"1983",
  editor = 	"Cutler, A. and Ladd, D.~Robert",
  OPTchapter = 	"",
  pages = 	"11-26",
  OPTaddress = 	"Berlin",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Gazdar80b,
  author = 	"Gazdar, Gerald",
  title = 	"Pragmatic Constraints on Linguistic Production",
  booktitle = 	"Language Production",
  publisher = 	ac,
  year = 	"1980",
  editor = 	"Butterword, B.",
  OPTchapter = 	"",
  pages = 	"49-68",
  OPTaddress = 	ny,
  OPTmonth = 	"",
  note = 	"Vol. 1:  Speech and Talk"
}

@Article{Gee83,
  author = 	"Gee, J.~ P.~ and F.~ Grosjean",
  title = 	"Performance Structure: A Psycholinguistic and
		 Linguistic Apprasial",
  journal = 	"Cognitive  Psychology",
  year = 	"1983",
  volume = 	"15",
  OPTnumber = 	"",
  pages = 	"411--458",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Gibbon84,
  OPTauthor = 	"",
key = "Gibbon",
  title = 	"Intonation, Accent, and Rhythm:  Studies in Discourse Phonology",
  publisher = 	"Walter de Gruyter",
  year = 	"1984",
  editor = 	"D.~Gibbon and H.~Richter",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Berlin",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Gleitman61,
  author = 	"Gleitman, L.",
  title = 	"Pronominals and Stress in {E}nglish",
  journal = 	"Language Learning",
  year = 	"1961",
  volume = 	"11",
  OPTnumber = 	"",
  pages = 	"157-169",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Goodwin81,
  author = 	"Goodwin, C.",
  title = 	"Conversational Organization:  Interaction between
		 Speakers and Hearers",
  publisher = 	ac,
  year = 	"1981",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	ny,
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Grosjean79,
  author = 	"Grosjean, F. and Grosjean, L. and Lane, H.",
  title = 	"The Patterns of Silence:  Performance Structures in
		 Sentence Production",
  journal = 	"Cognitive Psychology",
  year = 	"1979",
  volume = 	"11",
  OPTnumber = 	"",
  pages = 	"58-81",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Grosjean87,
  author = 	"Grosjean, F. and Gee, J.~P.",
  title = 	"Prosodic Structure and Spoken Work Recognition",
  journal = 	"Cognition",
  year = 	"1987",
  volume = 	"25",
  OPTnumber = 	"",
  pages = 	"135-155",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Grosz92,
  author = 	"Grosz, B. and Hirschberg, J.",
  title = 	"Some Intonational Characteristics of
Discourse Structure",
  booktitle = 	"Proceedings of the International Conference on
Spoken Language Processing",
  year = 	"1992",
  OPTeditor = 	"",
  OPTpages = 	"",
  organization = 	"ICSLP",
  OPTpublisher = 	"",
  address = 	"Banff",
  month = 	"October",
  OPTnote = 	""
}

@InCollection{Gumperz77,
  author = 	"Gumperz, J.~J.",
  title = 	"Sociocultural Knowledge in Conversational Inference",
  booktitle = 	"Linguistics and Anthropology",
  publisher = 	"Georgetown University Press",
  year = 	"1977",
  editor = 	"Saville-Troike, M.",
  OPTchapter = 	"",
  pages = 	"191-211",
  address = 	"Washington",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Gundel78,
  author = 	"Gundel, J.",
  title = 	"Stress, Pronominalization, and the Given-New Distinction",
  journal = 	"University of Hawaii Working Papers in Linguistics",
  year = 	"1978",
  volume = 	"10",
  number = 	"2",
  pages = 	"1-13",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Gussenhoven83a,
	Author="Gussenhoven, Carlos",
	Key="Gussenhoven",
	Title="On the Grammar and Semantics of Sentence Accents",
	Publisher=foris,
	Address="Dordrecht",
	Year="1983"}

@Book{Halliday67b,
  author = 	"Halliday, M.~A.~K.",
  title = 	"Intonation and Grammar in British {E}nglish",
  publisher = 	"Mouton",
  year = 	"1967",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"The Hague",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Halliday76,
  author = 	"Halliday, M.~A.~K. and Hassan, Ruquaiya",
  title = 	"Cohesion in {E}nglish",
  publisher = 	"Longman",
  year = 	"1976",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  OPTaddress = 	"",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Harries-Delisle78,
  author = 	"Harries-Delisle, H.",
  title = 	"Contrastive Emphasis and Cleft sentences",
  booktitle = 	"Universals of Human Language",
  publisher = 	stanfordp,
  year = 	"1978",
  editor = 	"Greenberg, J.",
  OPTchapter = 	"",
  pages = 	"419-486",
  OPTaddress = 	"Stanford",
  OPTmonth = 	"",
  OPTnote = 	"Vol. 4:  Syntax"
}

@Inproceedings{Hemphill90,
  author = 	"Hemphill, Charles T and Godfrey, John J. and
		 Doddington, George R..",
  title = 	"The ATIS Spoken Language Systems Pilot Corpus",
  booktitle = 	"Proceedings of the Speech and Natural Language Workshop",
  year = 	"1990",
  organization = "{DARPA}",
  pages = 	"96-101",
  address = 	"Hidden Valley PA",
  month = 	"June",
  OPTnote = 	""
}

@inproceedings{Hirschberg86,
	author="Hirschberg, J. and Pierrehumbert, J.",
	title="The Intonational Structuring of Discourse",
	booktitle="Proceedings of the 24th Annual Meeting",
	organization=acl,
	address=ny,
	year="1986",
	pages="136-144"}

@inproceedings{Hirschberg87a,
	author="Hirschberg, Julia and Litman, Diane",
	title="Now Let's Talk about {\em Now}: Identifying Cue Phrases
		Intonationally",
	booktitle="Proceedings of the 25th Annual Meeting",
	organization=acl,
	address=stanford,
        pages="163-171",
	year="1987"}

@InCollection{Hirschberg89,
  author = 	"Hirschberg, Julia",
  title = 	"Distinguishing Questions by Contour in Speech
		 Recognition Tasks",
  booktitle = 	"Proceedings of the Speech and Natural Language Workshop",
  publisher = 	"Morgan Kaufmann",
  year = 	"1989",
  organization = "{DARPA}",
  OPTchapter = 	"",
  OPTpages = 	"22-33",
  address = 	"Cape Cod MA",
  month = 	"October",
  OPTnote = 	""
}

@inproceedings{Hirschberg90,
	key="Hirschberg",
	author="Hirschberg, J.~",
	title="Accent and Discourse Context:  Assigning Pitch Accent
		 in Synthetic Speech",
        booktitle="Proceedings of the Eighth National Conference",
        organization=aaai,
        address="Boston",
        pages="952-957",
        year="1990"}

@InProceedings{Hirschberg90a,
  author = 	"Hirschberg, J.~",
  title = 	"Using Discourse Context to Guide Pitch Accent Decisions in
Synthetic
Speech",
  booktitle = 	"Proceedings of the {E}uropean Speech Communication Association
Workshop on Speech Synthesis",
  OPTpublisher = 	"",
  year = 	"1990",
  OPTeditor = 	"",
  OPTchapter = 	"",
  organization = 	"{E}uropean Speech Communication Association",
  pages = 	"181-184",
  address = 	"Autrans, France",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Hirschberg91a,
  author = 	"Hirschberg, J.~ and Ward, G.~",
  title = 	"Accent and Bound Anaphora",
  journal = 	"Cognitive Linguistics",
  year = 	"1991",
  volume = 	"2",
  number = 	"2",
  pages = 	"101--121",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Hirschberg91b,
  author = 	"Hirschberg, J.~ and Ward, G.~",
  title = 	"The Influence of Pitch Range, Duration, Amplitude,
		 and Spectral Features on the Interpretation of {\bf
		 L*+H L H\%}",
  journal = 	"Journal of Phonetics",
  year = 	"1991",
  OPTvolume = 	"",
  OPTnumber = 	"",
  OPTpages = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Hirschberg92b,
  author = 	"Hirschberg, J.~ and B.~ Grosz",
  title = 	"Intonational Features of Local and Global Discourse Structure",
  booktitle = 	"Proceedings of the  Speech and Natural Language Workshop",
  year = 	"1992",
  OPTeditor = 	"",
  pages = 	"441-446",
  organization = "DARPA",
  publisher = "Morgan Kaufmann",
  address = 	"Harriman NY",
  month = 	"February",
  OPTnote = 	""
}

@Misc{Hirsh-Pasek85,
  author = 	"Hirsh-Pasek, K. and D. Kemler Nelson and P. Jusczyk
		 and K. Wright and B. Druss",
  title = 	"Clauses are Perceptual Units for Prelinguistic Infants",
  howpublished = 	"Paper presented at the Tenth Annual Boston
		 University Conference on Language Development",
  year = 	"1985",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Hirst83,
  author = 	"Hirst, D.",
  title = 	"Structures and Categories in Prosodic Representations",
  booktitle = 	"Prosody:  Models and Measurements",
  publisher = 	sv,
  year = 	"1983",
  editor = 	"Cutler, A. and Ladd, D.~Robert",
  OPTchapter = 	"",
  pages = 	"93-110",
  address = 	"Berlin",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Horne85,
  author = 	"Horne, M.",
  title = 	"{E}nglish Sentence Stress, Grammatical Functions and
		 Contextual Coreference",
  journal = 	"Studia Linguistica",
  year = 	"1985",
  volume = 	"39",
  OPTnumber = 	"",
  pages = 	"51-66",
  OPTmonth = 	"",
  OPTnote = 	""
}

@TechReport{Horne87,
  author = 	"Horne, Merle",
  title = 	"Towards a Discourse-Based Model of {E}nglish Sentence Intonation",
  institution = "Lund University Department of Linguistics",
  year = 	"1987",
  type = 	"Working Papers",
  number = 	"32",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@TechReport{Horne91a,
  author = 	"Horne, M.",
  title = 	"Accentual Patterning in `New' vs `Given' Subjects in
		 {E}nglish",
  institution = 	"Department of Linguistics, Lund University",
  year = 	"1991",
  type = 	"Working Papers",
  number = 	"36",
  address = 	"Lund",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Horne91b,
  author = 	"Horne, M.",
  title = 	"Phonetic Correlates of the New/Given Parameter",
  booktitle = 	"Proceedings of the Twelfth International Congress of
		 Phonetic Sciences",
  year = 	"1991",
  OPTeditor = 	"",
  pages = 	"230-233",
  organization = 	"ICPhS",
  OPTpublisher = 	"",
  address = 	"Aix-en-Provence",
  OPTmonth = 	"",
  OPTnote = 	""
}

@TechReport{JHouse90a,
  author = 	"House, Jill",
  title = 	"A Revised Model for Intonation for Synthesis by Rule",
  institution = 	"University College London",
  year = 	"1990",
  type = 	"Speech, Hearing and Language:  Work in Progress",
  number = 	"U.~C.~L. No. 4",
  address = 	"London",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{JHouse90b,
  author = 	"House, Jill and Nick Youd",
  title = 	"Contextually Appropriate Intonation in Speech
		 Synthesis",
  booktitle = 	"Proceedings of the {E}uropean Speech Communication
		 Association
Workshop on Speech Synthesis",
  year = 	"1990",
  OPTeditor = 	"",
  pages = 	"185-188",
  organization = 	"{E}uropean Speech Communication Association",
  OPTpublisher = 	"",
  address = 	"Autrans",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Jackendoff72,
	Author="Jackendoff, Ray ~S.",
	Key="Jackendoff",
	Title="Semantic Interpretation in Generative Grammar",
	Publisher=mitp,
	Address="Cambridge MA",
	Year="1972"}

@Article{Klatt75a,
  author = 	"Klatt, D.",
  title = 	"Vowel Lengthening is Syntactically Determined in
		 Connected Discourse",
  journal = 	"Journal of Phonetics",
  year = 	"1975",
  volume = 	"3",
  OPTnumber = 	"",
  pages = 	"129-140",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Klatt87,
  author = 	"Klatt, Dennis H.",
  title = 	"Review of Text-to-Speech Conversion for {E}nglish",
  journal = 	jasa,
  year = 	"1987",
  volume = 	"82",
  number = 	"3",
  pages = 	"737-793",
  OPTmonth = 	"",
  OPTnote = 	""
}

@PhDThesis{Kruyt85,
  author = 	"Kruyt, J.~G.",
  title = 	"Accents from Speakers to Listeners:  An Experimental
		 Study of the Production and Perception of Accent
		 Patterns in {D}utch",
  school = 	"University of Leyden",
  year = 	"1985",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Kumpf87,
  author = 	"Kumpf, Lorraine E.",
  title = 	"The Use of Pitch Phenomena in the Structuring of
		 Stories",
  booktitle =   "Coherence and Grounding in Discourse",
  publisher = 	"John Benjamins Publishing Company",
  year = 	"1987",
  editor = 	"Tomlin, R.~S.",
  OPTpages = 	"189-216",
  volume = 	"11",
  OPTseries = 	"Typology Studies in Language",
  OPTaddress = 	"",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Kutik83,
  author = 	"Kutik, E.~J. and Cooper, W.~E. and Boyce, S.",
  title = 	"Declination of Fundamental Frequency in Speaker's
		 Production of Parenthetical and Main Clauses",
  journal = 	jasa,
  year = 	"1983",
  volume = 	"73",
  OPTnumber = 	"",
  pages = 	"1731-1738",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{LWitten77,
  author = 	"Witten, L. and Madams, P.",
  title = 	"The Telephone Inquiry Service:  A Man-Machine System
		 Using Synthetic Speech",
  journal = 	"International Journal of Man-Machine Studies",
  year = 	"1977",
  volume = 	"9",
  OPTnumber = 	"",
  pages = 	"449-464",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Unpublished{Ladd77,
  author = 	"Ladd, D.~Robert",
  title = 	"The Function of the A-Rise Accent in {E}nglish",
  note = 	"Distributed by the Indiana University Linguistics Club",
  year = 	"1977",
  OPTmonth = 	""
}

@Article{Ladd78,
  author = 	"Ladd, D.~Robert",
  title = 	"Stylized Intonation",
  journal = 	"Language",
  year = 	"1978",
  volume = 	"54",
  OPTnumber = 	"",
  pages = 	"517-540",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Ladd80,
	Author="Ladd, D. Robert",
	Key="Ladd",
	Title="The Structure of Intonational Meaning",
	Publisher="Indiana University Press",
	Address="Bloomington, Ind.",
	Year="1980"}

@InCollection{Ladd83a,
  author = 	"Ladd, D.~Robert",
  title = 	"Peak Features and Overall Slope",
  booktitle = 	"Prosody:  Models and Measurements",
  publisher = 	sv,
  year = 	"1983",
  editor = 	"Cutler, A. and Ladd, D.~Robert",
  OPTchapter = 	"",
  pages = 	"39-52",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Ladd83b,
  author = 	"Ladd, D.~Robert",
  title = 	"Phonological Features of Intonational Peaks",
  journal = 	lang,
  year = 	"1983",
  volume = 	"4",
  OPTnumber = 	"",
  pages = 	"721-759",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Ladd83c,
  author = 	"Ladd, D.~Robert",
  title = 	"Levels-vs.-Configurations, Revisited",
  booktitle = 	"Essays in Honor of Charles F. Hockett",
  publisher = 	"E.~J.~Brill",
  year = 	"1983",
  editor = 	"Agard et al",
  OPTchapter = 	"",
  OPTpages = 	"",
  address = 	"Leiden",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Ladd85,
  author = 	"Ladd, D.~R. and K.~E.~A.~Silverman and F.~Tolkmitt
		 and G.~Bergmann and K.~R.~Scherer",
  title = 	"Evidence for the Independent Function of Intonation
		 Contour Type, Voice Quality, and F0 Range in
		 Signaling Speaker Affect",
  journal = 	jasa,
  year = 	"1985",
  volume = 	"78",
  number = 	"1",
  pages = 	"435-444",
  month = 	"August",
  OPTnote = 	""
}

@Article{Ladd86,
  author = 	"Ladd, D. Robert",
  title = 	"Intonational Phrasing:  The Case for Recursive
		 Prosodic Structure",
  journal = 	"Phonology Yearbook",
  year = 	"1986",
  volume = 	"3",
  OPTnumber = 	"",
  pages = 	"311-340",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Ladd87a,
  author = 	"Ladd, D.~R. and Monaghan, A.",
  title = 	"Modelling Rhythmic and Syntactic Effects on Accent in
		 Long Noun Phrases",
  booktitle = 	"Proceedings of the {E}uropean Conference on Speech Technology",
  year = 	"1987",
  editor = 	"Laver, J.~ and M.~ Jack",
  publisher = 	"{CEP}",
  pages = 	"29--32",
  address = 	"Edinburgh",
  OPTaddress = 	"",
  OPTmonth = 	"",
}

@Article{Ladd88,
  author = 	"Ladd, D. Robert",
  title = 	"Declination `Reset' and the Hierarchical Organization
		 of Utterances",
  journal = 	jasa,
  year = 	"1988",
  volume = 	"84",
  OPTnumber = 	"",
  pages = 	"530-544",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Ladefoged62,
  author = 	"Ladefoged, Peter",
  title = 	"Elements of Acoustic Phonetics",
  publisher = 	"The University of Chicago Press",
  year = 	"1962",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Chicago",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@incollection{Lakoff71,
	key="Lakoff",
	author="Lakoff, George",
	title="Presupposition and Relative Well-Formedness",
	booktitle="Semantics:  An Interdisciplinary Reader in
Philosophy, Linguistics, and Psychology",
	editors="Steinberg, D. and Jakobovits, L.",
	year="1971",
	Publisher="Cambridge University Press",
	Address="Cambridge UK",
	pages="329-340"}

@Article{Lea75,
  author = 	"Lea, W. A. and Medress, M. F. and Skinner, T. E.",
  title = 	"A Prosodically Guided Speech Understanding System",
  journal = 	"IEEE Trans. Acoust. Speech, Signal Processing",
  year = 	"1975",
  volume = 	"ASSP-23",
  OPTnumber = 	"",
  pages = 	"30-38",
  month = 	"February",
  OPTnote = 	""
}

@incollection{Lea79,
	key="Lea",
	author="Lea, W.~A.",
	title="Prosodic Aids to Speech Recognition",
	booktitle="Trends in Speech Recognition",
	editor="Lea, W.~A.",
	publisher=ph,
	address="Englewood Cliffs NJ",
	year="1979",
	pages="166-205"}

@Article{Lehiste73,
  author = 	"Lehiste, I.",
  title = 	"Phonetic Disambiguation of Syntactic Ambiguity",
  journal = 	"Glossa",
  year = 	"1973",
  volume = 	"7",
  OPTnumber = 	"",
  pages = 	"197-222",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Lehiste76,
  author = 	"Lehiste, I. and Olive, J. and Streeter, L.",
  title = 	"Role of Duration in Disambiguating Syntactically
		 Ambiguous Sentences",
  journal = 	jasa,
  year = 	"1976",
  volume = 	"60",
  OPTnumber = 	"",
  pages = 	"1199-1202",
  OPTmonth = 	"",
  OPTnote = 	""
}

@article{Lehiste80a,
author="Lehiste, I.",
title="Phonetic Manifestation of Syntactic Structure in {E}nglish",
year="1980",
journal="Annual Bulletin of the Research Institute of Logopedics and
		 Phoniatrics, University of Tokyo",
volume="14",
number="1-27"
}

@Unpublished{Lehiste80b,
  author = 	"Lehiste, I.",
  title = 	"Phonetic Characteristics of Discourse",
  note = 	"Paper presented at the Meeting of the Committee on
		 Speech Research, Acoustical Society of {J}apan",
  year = 	"1980",
  OPTmonth = 	""
}

@InProceedings{Lehman77,
  author = 	"Lehman, C.",
  title = 	"A Re-analysis of Givenness:  Stress in Discourse",
  booktitle = 	"Papers from the 13th Annual Meeting",
  year = 	"1977",
  OPTeditor = 	"",
  pages = 	"316-",
  organization = 	cls,
  OPTpublisher = 	"",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Liberman74,
	Author="Liberman, Mark and Sag, Ivan A. ",
	Key="Liberman and Sag",
	Title="Prosodic Form and Discourse Function",
	Organization=cls,
	BookTitle="Papers of the Tenth Regional Meeting",
	Pages="416-427",
	Year="1974"}

@PhDThesis{Liberman75,
  author = 	"Liberman, Mark Y.",
  title = 	"The Intonation System of {E}nglish",
  school = 	"MIT",
  year = 	"1975",
  address = 	"Cambridge MA",
  OPTmonth = 	""
}

@Article{Liberman77,
	Author="Liberman, Mark and Alan Prince",
	Key="Liberman",
	Title="On Stress and Linguistic Rhythm",
	Journal="Linguistic Inquiry",
	Volume="8",
	Number="2",
        Pages="249-336",
	Year="1977"}

@incollection{Liberman84,
	key="Liberman",
	author="Liberman, M. and Pierrehumbert, J.",
	title="Intonational Invariants under Changes in Pitch Range and Length",
	booktitle="Language Sound Structure",
	editor="Aronoff, M. and Oehrle, R.",
	publisher="MIT Press",
	address="Cambridge",
	year="1984"}

@InProceedings{Litman90,
  author = 	"Litman, Diane and Hirschberg, Julia",
  title = 	"Disambiguating Cue Phrases in  Text and Speech",
  booktitle = 	coling90,
  year = 	"1990",
  OPTeditor = 	"",
  pages = 	"251-256",
  organization = 	coling,
  OPTpublisher = 	"",
  address = 	"Helsinki",
  month = 	"August",
  OPTnote = 	""
}

@PhDThesis{Ljolje86,
  author = 	"Ljolje, Andrej",
  title = 	"Intonation and Phonetic Segmentation Using Hidden
		 Markov Models",
  school = 	"University of Cambridge",
  year = 	"1986",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Ljolje87a,
  author = 	"Ljolje, Andrej and Frank Fallside",
  title = 	"Modelling of Speech Using Primarily Prosodic Parameters",
  journal = 	"Computer Speech and Language",
  year = 	"1987",
  volume = 	"2",
  OPTnumber = 	"",
  pages = 	"185-204",
  OPTmonth = 	"",
  OPTnote = 	""
}

@inproceedings{Lujan85,
	key="Lujan",
	author="Luj\'{a}n, Marta",
	title="Stress and the Binding of Pronouns",
	organization=cls,
	booktitle="Papers of the Twenty-first Regional Meeting",
	year="1985",
	pages="248-262"}

@inproceedings{Marcus85,
	key="Marcus",
	author="Marcus, Mitchell P. and Donald Hindle",
	year="1985",
	title=" A Computational Account of Extra Categorial Elements
in {J}apanese",
	booktitle="Papers presented at the First SDF Workshop
in {J}apanese Syntax",
        address="La Jolla",
        editor="S. Y. Kuroda",
	organization="System Development Foundation"}

@incollection{Marcus90,
author = "Marcus, Mitchell P. and Donald Hindle",
year = "1990",
title = "Description Theory and Intonation Boundaries",
booktitle="Computational
and Cognitive Models of Speech",
editor= "Gerald Altmann",
publisher=mitp,
address=cambma}

@Article{Martin70,
  author = 	"Martin, E.",
  title = 	"Toward an Analysis of Subjective Phrase Structure",
  journal = 	"Psychological Bulletin",
  year = 	"1970",
  volume = 	"74",
  OPTnumber = 	"",
  pages = 	"153-166",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Misono90,
  author = 	"Misono, Yasuko and Kiritani, Shigeru",
  title = 	"The Distribution Pattern of Pauses in Lecture-Style Speech",
  journal = 	"Annual Bulletin of the RILP",
  year = 	"1990",
  volume = 	"24",
  OPTnumber = 	"24",
  pages = 	"101-111",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Morgan87,
  author = 	"Morgan, J.~L.~ and R.~P.~ Meier and E.~L.~ Newport",
  title = 	"Structural Packaging in the Input to Language
		 Learning:  Contributions of Prosodic and
		 Morphological Marking of Phrases to the Acquisition
		 of Language",
  journal = 	"Cognitive Psychology",
  year = 	"1987",
  volume = 	"19",
  OPTnumber = 	"",
  pages = 	"498-550",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Nash80,
  author = 	"Nash, Rose and Mulac, Anthony",
  title = 	"The Intonation of Verifiability",
  booktitle = 	"The Melody of Language",
  publisher = 	"University Park Press",
  year = 	"1980",
  editor = 	"Waugh, L.~R. and C.~H. van Schooneveld",
  OPTchapter = 	"",
  pages = 	"219-242",
  address = 	"Baltimore",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Nooteboom82,
  author = 	"Nooteboom, S.~G. and J.~Terken",
  title = 	"What Makes Speakers Omit Pitch Accents?:  An Experiment",
  journal = 	"Phonetica",
  year = 	"1982",
  volume = 	"39",
  OPTnumber = 	"",
  pages = 	"317-336",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{O'Connor61,
	Author="O'Connor, J.D. and Arnold, G.F.",
	Key="O'Connor",
	Title="Intonation of Colloquial {E}nglish",
	Publisher="Longman",
	Address="London",
	Year="1961"}

@Article{O'Malley73,
  author = 	"O'Malley, M. M. and Kloker, D. and Dara-Abrams, B.",
  title = 	"Recovering Parentheses from Spoken Algebraic Expressions",
  journal = 	"IEEE Trans. Audio Electroacoust.",
  year = 	"1973",
  volume = 	"AU-21",
  OPTnumber = 	"",
  pages = 	"217-220",
  month = 	"June",
  OPTnote = 	""
}

@Article{O'Shaughnessy89,
  author = 	"O'Shaughnessy, D.",
  title = 	"Parsing with a Small Dictionary for Applictions such
		 as Text to Speech",
  journal = 	"Computational Linguistics",
  year = 	"1989",
  volume = 	"15",
  number = 	"2",
  pages = 	"97-108",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Oakeshott84,
  author = 	"Oakeshott-Taylor, John",
  title = 	"Factuality and Intonation",
  journal = 	"Journal of Linguistics",
  year = 	"1984",
  volume = 	"20",
  OPTnumber = 	"",
  pages = 	"1-21",
  OPTmonth = 	"",
  OPTnote = 	""
}

@article{Olive85,
	key="Olive",
	author="Olive, J. P. and Liberman, M. Y.",
	title="Text to speech -- An overview",
	journal="Journal of the Acoustic Society of America, Suppl. 1",
	volume="78",
	number="Fall",
	year="1985",
	pages="s6"}

@Inproceedings{Ostendorf90,
  author = 	"Ostendorf, M. and Price, P. and Bear, J. and
		 Wightman, C. W.",
  title = 	"The Use of Relative Duration in Syntactic Disambiguation",
  booktitle = 	"Proceedings of the Speech and Natural Language Workshop",
  publisher = 	"Morgan Kaufmann",
  year = 	"1990",
  organization = "{DARPA}",
  pages = 	"26-31",
  address = 	"Hidden Valley PA",
  month = 	"June",
  OPTnote = 	""
}

@PhDThesis{Pierrehumbert80,
	Author="Pierrehumbert, Janet B.",
	Key="Pierrehumbert",
	Title="The Phonology and Phonetics of {E}nglish Intonation",
	School="Massachusetts Institute of Technology",
	Month="September",
	Year="1980",
        note="Distributed by the Indiana University Linguistics Club"}

@Article{Pierrehumbert81,
  author = 	"Pierrehumbert, J.",
  title = 	"Synthesising Intonation",
  journal = 	jasa,
  year = 	"1981",
  volume = 	"70",
  number = 	"4",
  pages = 	"985-995",
  OPTmonth = 	"",
  OPTnote = 	""
}

@inproceedings{Pierrehumbert83,
	key="Pierrehumbert",
	author="Pierrehumbert, Janet B.",
	title="Automatic Recognition of Intonation Patterns",
	booktitle="Proceedings of the 21st Annual Meeting",
	organization=acl,
	address="Cambridge MA",
	year="1983",
	pages="85-90"}

@inproceedings{Pierrehumbert87b,
	key="Pierrehumbert",
	author="Pierrehumbert, Janet B. and Steele, Shirley",
	title="How Many Rise-Fall-Rise Contours?",
	booktitle="Proceedings of the Eleventh Meeting",
	organization="International Congress of Phonetic Sciences",
	year="1987",
	address="Tallinn"}

@Article{Pierrehumbert89,
  author = 	"Pierrehumbert, Janet",
  title = 	"Categories of Tonal Alignment in {E}nglish",
  journal = 	"Phonetica",
  year = 	"1989",
  OPTvolume = 	"",
  OPTnumber = 	"",
  OPTpages = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@incollection{Pierrehumbert90,
	key="Pierrehumbert",
	author="Pierrehumbert, Janet and Hirschberg, Julia",
	title="The Meaning of Intonational Contours in the
Interpretation of Discourse",
	editor="Cohen, P. and Morgan, J. and Pollack, M.",
	booktitle="Intentions in Communication",
	publisher=mitp,
	year="1990",
	address="Cambridge MA"}

@Book{Pike45,
	Author="Pike, Kenneth",
	Key="Pike",
	Title="The Intonation of {American} {{E}nglish}",
	Publisher="University of Michigan Press",
	Address="Ann Arbor MI",
	Year="1945"}

@inproceedings{Price88,
	key="Price",
	author="Price, P. and Fisher, W.~M. and Bernstein, J. and
		Pallett, D.~S.",
	title="The {{DARPA}} 1000-Word {R}esource {M}anagement {D}atabase for
		Continuous Speech Recognition",
	booktitle="Proceedings",
	organization="ICASSP88",
	address=ny,
	year="1988",
	pages="651-654",
	volume="1"}

@InCollection{Prince84,
  author = 	"Prince, E.~F.",
  title = 	"Language and the Law:  Reference, Stress, and Context",
  booktitle = 	"GURT84:  Meaning, Form and Use in Context:
		 Linguistic Applications",
  publisher = 	"Georgetown University Press",
  year = 	"1984",
  editor = 	"Schiffrin, D.",
  OPTchapter = 	"",
  pages = 	"240-252",
  address = 	"Washington DC",
  OPTmonth = 	"",
  OPTnote = 	""
}

@inproceedings{Quirk64,
	key="Quirk",
	author="Quirk, R. and Svartvik, J. and Duckworth, A. P. and
Rusiecki,J. P. L.
and Colin, A. J. T.",
	title="Studies in the Correspondence of Prosodic to
Grammatical Features in {E}nglish",
	organization="International Congress of Linguists",
	booktitle="Proceedings of the Ninth International Congress",
	year="1964",
	pages="679-691"}

@Article{Ratner86,
  author = 	"Ratner, Nan Bernstein",
  title = 	"Durational Cues which Mark Clause Boundaries in
		 Mother-Child Speech",
  journal = 	"Journal of Phonetics",
  year = 	"1986",
  volume = 	"14",
  OPTnumber = 	"",
  pages = 	"303-309",
  OPTmonth = 	"",
  OPTnote = 	""
}

@TechReport{Rees76,
  author = 	"Rees, M. and Urquhart, A.~H.",
  title = 	"Intonation as a Guide to Readers' Structuring of
		 Prose Texts",
  institution = 	"University of Edinburgh",
  year = 	"1976",
  type = 	"Work in Progress",
  number = 	"9",
  address = 	"Department of Linguistics",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{Rochemont90,
  author = 	"Rochemont, Michael S. and Peter W. Culicover",
  title = 	"{E}nglish Focus Constructions and the Theory of Grammar",
  publisher = 	"Cambridge University Press",
  year = 	"1990",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Cambridge UK",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Roe91,
  author = 	"Roe, David B.~ and Pereira, Fernando and Sproat,
		 Richard W.~ and Riley, Michael D.~ and Moreno, Pedro
		 J.~ and Macarron, Alejandro",
  title = 	"Toward a Spoken Language Translator for
		 Restricted-Domain Context-Free Languages",
  booktitle = 	"Proceedings of the Second {E}uropean Conference on
		 Speech Communication and Technology",
  year = 	"1991",
  OPTeditor = 	"",
  pages = 	"1063--1066",
  organization = 	"Eurospeech-91",
  OPTpublisher = 	"",
  address = 	"Genova",
  month = 	"September",
  OPTnote = 	""
}

@phdthesis{Rooth85,
	author="Rooth, Mats",
	title="Association with Focus",
	key="Rooth",
	school="University of Massachusetts",
	address="Amherst MA",
	year="1985"}

@Misc{Rooth91,
  author = 	"Rooth, Mats",
  title = 	"A Theory of Focus Interpretation",
  howpublished = 	"Presented at the Workshop on the Syntax
		 and Semantics of Focus, Third {E}uropean Summer School
		 in Language, Logic and Information, Universitaet des
		 Saarlandes, Saarbrucken",
  year = 	"1991",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Sag75,
  author = 	"Sag, I.~A.~ and Liberman<, M.~Y.~",
  title = 	"The Intonational Disambiguation of Indirect Speech Acts",
  booktitle = 	"Papers from the Eleventh Regional Meeting",
  year = 	"1975",
  OPTeditor = 	"",
  OPTpages = 	"",
  organization = 	cls,
  OPTpublisher = 	"",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Schegloff79b,
  author = 	"Schegloff, E.~A.",
  title = 	"Identification and Recognition in Telephone
		 Conversation Openings",
  booktitle = 	"Everyday Language:  Studies in Ethnomethodology",
  publisher = 	"Irvington",
  year = 	"1979",
  editor = 	"Psathas, G.",
  OPTchapter = 	"",
  pages = 	"23-78",
  address = 	ny,
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Scherer84,
  author = 	"Scherer, Klaus and Ladd, D. Robert and Silverman, Kim
		 E. A.",
  title = 	"Vocal Cues to Speaker Affect:  Testing Two Models",
  journal = 	jasa,
  year = 	"1984",
  volume = 	"76",
  number = 	"5",
  pages = 	"1346-1356",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Schmerling71,
  author = 	"Schmerling, S.",
  title = 	"Presupposition and the Notion of Normal Stress",
  booktitle = 	"Papers from the 7th Regional Meeting",
  year = 	"1971",
  organization = cls,
  pages = 	"242-253",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Schmerling74,
  author = 	"Schmerling, S.",
  title = 	"A Re-examination of the Notion {NORMAL STRESS}",
  journal = 	lang,
  year = 	"1974",
  volume = 	"50",
  OPTnumber = 	"",
  pages = 	"66-73",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Schmerling75b,
  author = 	"Schmerling, S.",
  title = 	"Evidence from Sentence Stress for the Notions of
		 Topic and Comment",
  booktitle = 	"Texas Linguistics Forum",
  publisher = 	"University of Texas",
  year = 	"1975",
  editor = 	"Schmerling, S. and King, R.",
  OPTchapter = 	"",
  pages = 	"135-141",
  address = 	"Department of Linguistics",
  OPTmonth = 	"",
  OPTnote = 	""
}

@book{Schmerling76,
	author="Schmerling, Susan F.",
	title="Aspects of {E}nglish Sentence Stress",
	publisher="University of Texas Press",
	address="Austin",
	year="1976",
	note="Revised 1973 thesis, University of Illinois at Urbana"}

@book{Selkirk84a,
	key="Selkirk",
	author="Selkirk, E.",
	title="Phonology and Syntax",
	address=cambma,
	publisher=mitp,
	year="1984"}

@InCollection{Silva-Corvalan83,
  author = 	"Silva-Corvalan, C.",
  title = 	"On the Interaction of Word Order and Intonation:
		 Some {OV} Constructions in Spanish",
  booktitle = 	"Discourse Perspectives on Syntax",
  publisher = 	ac,
  year = 	"1983",
  editor = 	"Klein, F.",
  OPTchapter = 	"",
  pages = 	"117-140",
  OPTaddress = 	ny,
  OPTmonth = 	"",
  OPTnote = 	""
}

@inproceedings{Silverman86,
	author="Silverman, K.",
	title="Synthesis and Perception of Paragraph Prosody",
	organization="First Australian Conference of Speech Science
and Technology",
	booktitle="Proceedings",
	year="1986"}

@phdthesis{Silverman87,
	author="Silverman, K.",
	title="The Structure and Processing of Fundamental Frequency Contours",
	school="Cambridge University",
	year="1987",
	address="Cambridge UK"}

@InProceedings{Silverman92a,
  author = 	"Silverman, Kim E.~ A.~ and Eleonora Blaauw and Judith
		 Spitz and John F.~ Pitrelli",
  title = 	"Towards using Prosody in Speech
		 Recognition/Understanding Systems: Differences
		 between Read and Spontaneous Speech",
  booktitle = 	"Proceedings of the Speech and
		 Natural Language Workshop",
  year = 	"1992",
  OPTeditor = 	"",
  pages = 	"435-440",
  organization = 	"DARPA",
  publisher = 	"Morgan Kaufmann",
  address = 	"Harriman NY",
  month = 	"February",
  OPTnote = 	""
}

@InProceedings{Sproat90,
  author = 	"Sproat, Richard",
  title = 	"Stress Assignment in Complex Nominals for {E}nglish
Text-to-Speech",
  booktitle = 	"Proceedings of the {E}uropean Speech Communication
		 Association
Workshop on Speech Synthesis",
  year = 	"1990",
  OPTeditor = 	"",
  pages = 	"129--132",
  organization = 	"{E}uropean Speech Communication Association",
  OPTpublisher = 	"",
  address = 	"Autrans, France",
  month = 	"September",
  OPTnote = 	""
}

@Inproceedings{Steedman90,
  author = 	"Steedman, M.",
  title = 	"Structure and Intonation in Spoken Language Understanding",
  booktitle = 	"Proceedings of the 28th Annual Meeting",
  year = 	"1990",
  OPTeditor = 	"",
  OPTchapter = 	"",
  pages =	 "9-16",
  address =	 "Pittsburgh",
organization = acl,
  OPTmonth = 	"",
  OPTnote = 	""
}

@article{Stockwell71,
	key="Stockwell",
	author="Stockwell, R.~P.",
	title="The Role of Intonation:  Reconsiderations and Other
Considerations",
	year="1971",
	journal="UCLA Working Papers in Phonetics",
	volume="21",
	pages="25-49",
	note="Cited in \cite{Schmerling76}"}

@Article{Streeter78,
  author = 	"Streeter, Lynn",
  title = 	"Acoustic Determinants of Phrase Boundary Perception",
  journal = 	jasa,
  year = 	"1978",
  volume = 	"63",
  number = 	"6",
  pages = 	"1582-1592",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Sugito90,
  author = 	"Sugito, Miyoko and Ohyama, Ghen and Hirose, Hajime",
  title = 	"A Preliminary Study on Pauses and Breaths in Reading
		 Speech Materials",
  journal = 	"Annual Bulletin of the RILP",
  year = 	"1990",
  volume = 	"24",
  OPTnumber = 	"24",
  pages = 	"121-130",
  OPTmonth = 	"",
  OPTnote = 	""
}

@PhDThesis{Taft84,
  author = 	"Taft, Lori",
  title = 	"Prosodic Constraints and Lexical Parsing Strategies",
  school = 	"University of Massachusetts",
  year = 	"1984",
  address = 	"Amherst MA",
  OPTmonth = 	"",
  OPTnote = 	""
}

@article{Talkin89,
	key="Talkin",
	author="Talkin, David",
	title="Looking at Speech",
	journal="Speech Technology",
	volume="4",
	month="April-May",
	year="1989",
	pages="74-77"}

@Article{Taylor87,
  author = 	"Taylor, Steven and Wales, Roger",
  title = 	"Primitive Mechanisms of Accent Perception",
  journal = 	"Journal of Phonetics",
  year = 	"1987",
  volume = 	"15",
  OPTnumber = 	"",
  pages = 	"235-246",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Terken84,
  author = 	"Terken, J.",
  title = 	"The Distribution of Pitch Accents in Instructions as
		 a Function of Discourse Structure",
  journal = 	"Language and Speech",
  year = 	"1984",
  volume = 	"27",
  OPTnumber = 	"",
  pages = 	"269-289",
  OPTmonth = 	"",
  OPTnote = 	""
}

@phdthesis{Terken85,
  author = 	"Terken, J.~M.~B.",
  title = 	"Use and Function of Accentuation:  Some Experiments",
  school="University of Leiden",
  address = 	"Helmond, Neth",
  year = 	"1985",
}

@Article{Terken87,
  author = 	"Terken, J. and S.~ G. Nooteboom",
  title = 	"Opposite Effects of Accentuation and Deaccentuation
		 on Verification Latencies for Given and New Information",
  journal = 	"Language and Cognitive Processes",
  year = 	"1987",
  volume = 	"2",
  number = 	"3/4",
  pages = 	"145-163",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Umeda82,
  author = 	"Umeda, N.",
  title = 	"Boundary:  Perceptual and Acoustic Properties and
		 Syntactic and Statistical Determinants",
  journal = 	"Speech and Language",
  year = 	"1982",
  volume = 	"7",
  OPTnumber = 	"",
  pages = 	"333-371",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Vaissiere83,
  author = 	"Vaissier, J.",
  title = 	"Language-Independent Prosodic Features",
  booktitle = 	"Prosody:  Models and Measurements",
  publisher = 	sv,
  year = 	"1983",
  editor = 	"Cutler, A. and Ladd, D.~Robert",
  OPTchapter = 	"",
  pages = 	"53-66",
  address = 	"Berlin",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Waibel79,
  author = 	"Waibel, A.",
  title = 	"The Pitch Contour in WH-questions",
  journal = 	"Speech Communication Papers",
  year = 	"1979",
  OPTvolume = 	"",
  OPTnumber = 	"",
  pages = 	"187-190",
  month = 	"June",
  note = 	"Acoustical Society of America"
}

@book{Waibel88,
	key="Waibel",
	author="Waibel, Alex",
	title="Prosody and Speech Recognition",
	publisher="Pitman Publishing",
	address="London",
	year="1988"}

@incollection{Lea79,
	key="Lea",
	author="Lea, W.~A.",
	title="Prosodic Aids to Speech Recognition",
	booktitle="Trends in Speech Recognition",
	editor="Lea, W.~A.",
	publisher=ph,
	address="Englewood Cliffs NJ",
	year="1979",
	pages="166-205"}

@Book{Waibel90a,
 title = 	"Readings in Speech Recognition",
  year = 	"1990",
  editor = 	"Waibel, A. and Lee, K.-F.",
  publisher = 	"Morgan Kaufmann Publishers, Inc.",
  address = 	"San Mateo CA",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InCollection{Wales79,
  author = 	"Wales, Roger and Toner, Hugh",
  title = 	"Intonation and Ambiguity",
  booktitle = 	"Sentence Processing:  Psycholinguistic Studies Presented to
Merrill Garrett",
  publisher = 	"Halsted Press",
  year = 	"1979",
  editor = 	"Cooper, W.~ E. and Walker, E.~C.",
  OPTchapter = 	"",
  OPTpages = 	"",
  address = 	ny,
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Wang91a,
  author = 	"Wang, Michelle Q. and Hirschberg, J.~",
  title = 	"Predicting Intonational Boundaries Automatically from
		 Text:  The {ATIS} Domain",
  booktitle = 	"Proceedings of the Speech and Natural Language Workshop",
  year = 	"1991",
  OPTeditor = 	"",
  pages = 	"378-383",
  organization = "{DARPA}",
  publisher = 	"Morgan Kaufmann",
  address = 	"Pacific Grove CA",
  month = 	"February",
  OPTnote = 	""
}

@Article{Wang92,
  author = 	"Wang, Michelle Q.~ and J.~ Hirschberg",
  title = 	"Automatic Classification of Intonational Phrase Boundaries",
  journal = 	"Computer Speech and Language",
  year = 	"1992",
  volume = 	"6",
  OPTnumber = 	"",
  pages = 	"175-196",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Ward85b,
	Author="Ward, G.~ and Hirschberg, J.~",
	Key="Ward",
	Title="Implicating Uncertainty:  The Pragmatics of Fall-Rise Intonation",
	Journal=lang,
        Volume="61",
	Number="4",
	Month="December",
        Pages="747-776",
	Year="1985"}

@TechReport{Wilkenfeld81,
  author = 	"Wilkenfeld, D.",
  title = 	"Reading, Prosody, and Orthography",
  institution = 	"Haskins Laboratories",
  year = 	"1981",
  type = 	"Status Report on Speech Research",
  number = 	"SR-67/68",
  OPTaddress = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Article{Williams80,
  author = 	"Williams, E.",
  title = 	"Remarks on Stress and Anaphora",
  journal = 	"Journal of Linguistic Research",
  year = 	"1980",
  volume = 	"1",
  number = 	"3",
  OPTpages = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}

@incollection{Wilson79,
	author="Wilson, Dierdre and Sperber, Dan",
	title="Ordered Entailments: An Alternative to Presuppositional Theories",
	booktitle="Syntax and Semantics",
	editor="Oh, C.-K. and Dinneen, D. A.",
	publisher=ac,
	address=ny,
	year="1979",
	volume="11",
	pages="229-324"}

@Article{Young79,
  author = 	"Young, S.~J. and Frank Fallside",
  title = 	"Speech synthesis from Concept:  A Method for Speech
		 Output from Information Systems",
  journal = 	"Journal of the Acoustic Society of America",
  year = 	"1979",
  volume = 	"66",
  number = 	"3",
  pages = 	"685-695",
  month = 	"September",
  OPTnote = 	""
}

@Article{Yule80,
  author = 	"Yule, G.",
  title = 	"Speakers' Topics and Major Paratones",
  journal = 	"Lingua",
  year = 	"1980",
  volume = 	"52",
  OPTnumber = 	"",
  pages = 	"33-47",
  OPTmonth = 	"",
  OPTnote = 	""
}

@InProceedings{Zacharski92,
  author = 	"Zacharski, Ron",
  title = 	"Generation of Accent in Nominally Premodified Noun Phrases",
  booktitle = 	coling92,
  year = 	"1992",
  OPTeditor = 	"",
  pages = 	"253--259",
  organization = 	coling,
  OPTpublisher = 	"",
  address = 	"Nantes",
  OPTmonth = 	"",
  OPTnote = 	""
}

@Book{tHart90,
  author = 	"J't. Hart and R. Collier and A. Cohen",
  title = 	"A Perceptual Study of Intonation",
  publisher = 	"Cambridge University Press",
  year = 	"1990",
  OPTeditor = 	"",
  OPTvolume = 	"",
  OPTseries = 	"",
  address = 	"Cambridge UK",
  OPTedition = 	"",
  OPTmonth = 	"",
  OPTnote = 	""
}



